The Writing is on the Wall: Analyzing the Boom of Inscriptions and its Impact on EVM-compatible Blockchains

This paper examines inscription-related transactions on Ethereum and major EVM-compatible rollups, assessing their impact on scalability during transaction surges. Our results show that, on certain days, inscriptions accounted for nearly 90% of transactions on Arbitrum and ZKsync Era, while 53% on Ethereum, with 99% of these inscriptions involving meme coin minting. Furthermore, we show that ZKsync and Arbitrum saw lower median gas fees during these surges. ZKsync Era, a ZK-rollup, showed a greater fee reduction than the optimistic rollups studied -- Arbitrum, Base, and Optimism.

==> Makefile <==
MAIN=main
SRCS=sections/*.tex

LMK=latexmk
OTYPE=-pdf
TEX=-pdflatex
TEX_OPTS="pdflatex -interaction=nonstopmode -shell-escape"
BIB=-bibtex

ERROR_MSG=Error: cannot find '$(LMK)' in path; try 'pdflatex $(MAIN).tex'

lmk_check =								\
	@which $(LMK) > /dev/null ||		\
		(echo "$(ERROR_MSG)" >& 2 &&	\
			exit 1)

default: $(MAIN).pdf

$(MAIN).pdf: $(MAIN).tex $(SRCS)
	$(call lmk_check)
	@$(LMK) $(OTYPE) $(TEX)=$(TEX_OPTS) $(BIB) $<

.PHONY: watch clean

# Automatically rebuild latex files whenever changes are made.
watch: $(MAIN).tex
	$(call lmk_check)
	@$(LMK) -pvc $(OTYPE) $(TEX)=$(TEX_OPTS) $(BIB) $<

clean:
	@rm -f *.dvi *.aux *.blg *.log *.ps *~ *.bbl *.fdb_latexmk *.fls $(MAIN).pdf *.out


==> sections/08_acknowledgments.tex <==
\section*{Acknowledgments}

This research article is a work of scholarship and reflects the authors' own views and opinions. It does not necessarily reflect the views or opinions of any other person or organization, including the authors' employer. Readers should not rely on this article for making strategic or commercial decisions, and the authors are not responsible for any losses that may result from such use.

